RHEEMix in the Data Jungle: A Cost-based Optimizer for Cross-platform Systems

In pursuit of efficient and scalable data analytics, the insight that "one size does not fit all" has given rise to a plethora of specialized data processing platforms and today's complex data analytics are moving beyond the limits of a single platform. In this paper, we present the cost-based optimizer of Rheem, an open-source cross-platform system that copes with these new requirements. The optimizer allocates the subtasks of data analytic tasks to the most suitable platforms. Our main contributions are: (i)~a mechanism based on graph transformations to explore alternative execution strategies; (ii)~a novel graph-based approach to efficiently plan data movement among subtasks and platforms; and (iii)~an efficient plan enumeration algorithm, based on a novel enumeration algebra. We extensively evaluate our optimizer under diverse real tasks. The results show that our optimizer is capable of selecting the most efficient platform combination for a given task, freeing data analysts from the need to choose and orchestrate platforms. In addition, our optimizer allows tasks to run more than one order of magnitude faster by using multiple platforms instead of a single platform.

==> background.tex <==
%!TEX root = main.tex

%\jorge{Henceforth, make sure that the reader understand that the effort from users to bootstrap the system is minimum: setting cost functions, cardinalities, bla, bla...}
%Before delving into the details of our cross-platform optimizer, let us briefly outline \rheem~\cite{rheem-demo} so as to establish the optimizer's context.
\rheem is a system that decouples data processing, \ie~separates applications from platforms, in order to enable cross-platform data processing.
%It acts as a unifying abstraction layer for co-existing platforms with the goal of enabling cross-platform data processing.
\add{Although decoupling data processing was the driving motive when designing \rheem, we also adopted a three-layer optimization approach envisioned in~\cite{rheem-vision}.
One can see this three-layer optimization as a separation of concerns for query optimization.
Overall, as \rheem applications have good knowledge of the tasks' logic and the data they operate on, they are in charge of any logical and physical optimizations, such as operator re-ordering (the application optimization layer). % and physical operator selection .
\rheem receives from applications an optimized procedural \rheem plan, for which it determines the best platforms for execution (the core optimization layer).
%Then, the \rheem optimizer translates a \rheem plan into an execution plan by deciding on which platform to execute each part of the \rheem plan (the core optimization layer).
Then, the selected platforms run the plan by performing further platform-specific optimizations, such as setting the data buffer sizes (the platform optimization layer).
In this paper, we focus on the core optimization layer.
}
% In Appendix~\ref{section:usecases}, we discuss the different cases in which applications either require or greatly benefit from cross-platform task processing.
%
%Figure~\ref{figure:architecture}\seb{We need to take good care to (i)~make the architecture not look too trivial, while (ii)~not distracting the reader or intriguing her too much \wrt~the other components of our system.}\zoi{I vote to remove the figure completely. I believe the text can stand on its own without the figure. Like this we can put a figure in the next figure for the optimizer that is the focus of this paper.} depicts the architecture of \rheem, which is composed of two main components: the {\em cross-platform optimizer} and the {\em executor}.
Among others, \rheem is composed of two main components: the {\em cross-platform optimizer} and the {\em executor}.
After detailing \add{what the input to the cross-platform optimizer is}, %how applications express their tasks, 
we briefly outline both components.
For more details about \rheem' architecture, we would like to refer the interested reader to~\cite{rheem-demo}.

%\begin{figure}[t!]
%	\centering
%	\includegraphics[width=0.75 \columnwidth]{figures/architecture}
%	\vspace{-0.3cm}
%	\caption{General \rheem architecture.}
%	\label{figure:architecture}
%	\vspace{-0.2cm}
%\end{figure}

\myparagraph{\rheem plan}
\add{The input to \rheem optimizer is a} %Applications send tasks to the system as 
	{\em \rheem plan}, which is essentially a directed data flow graph (\add{DG}).
%\seb{Can we reduce the set of synonymous terms \emph{query}, \emph{task}, \emph{plan}, and \emph{data flow graph}?}
%\jorge{I agree, but here we cannot do much: it is called like this DG}
The vertices are {\em \rheem operators} and the edges represent the data flow among the operators.
\add{Only} specific \at{Loop} operators accept feedback edges, thus enabling iterative data flows. \add{A \rheem plan without any loop operator is essentially an acyclic graph.}
Conceptually, the data is flowing from source operators through the \add{DG} and is manipulated in the operators until it reaches a sink operator.
%The atomic processing units flowing through the plan are called {\em data quanta}\zoi{let's keep it simpler and remove the data quanta term. We can replace it everywhere simply with data or data unit.} and can express a large spectrum of data formats, such as database tuples and graph edges.
\rheem operators are platform-agnostic and define a particular kind of data transformation over their input, \eg~a \at{Reduce} operator aggregates all input data into a single output.

\begin{figure}[!h]
	\vspace{-0.1cm}
	\centering
	\includegraphics[width=0.9 \columnwidth]{figures/rheemplan}
	\vspace{-0.4cm}
	\caption{K-means example.}
	\label{figure:plan}
	\vspace{-0.3cm}
\end{figure}

\vspace{-0.2cm}
\begin{example}
Figure~\ref{figure:plan}(a) shows a \rheem plan for k-means.
Data points are read via a \at{TextFileSource} and parsed using a \at{Map}, while the initial centroids are read via a \at{CollectionSource}.
The main operations of k-means (\ie~assigning the closest centroid to each data point and computing the new centroids) are repeated until convergence (\ie~the termination condition of \at{RepeatLoop}).
The resulting centroids are output in a collection.
To convey a tangible picture of the context in which our optimizer works, we present the actual code for this \rheem plan in Appendix~\ref{section:apps}.
%\seb{I suppose we should show and reference the code of that plan in the appendix (\eg~move up the last paragraph of this section).}
%\jorge{done: please check.}
\end{example}
\vspace{-0.2cm}

\myparagraph{Cross-platform optimizer ({\em focus of this paper})}
Given a \rheem plan, the optimizer determines how to best execute this plan.
That is, it produces an {\em execution plan} by selecting one or more data processing platforms as exemplified in Figure~\ref{figure:plan}(b).
The execution plan is again a data flow graph with two differences from a \rheem plan:
the vertices are (platform-specific) {\em execution operators}; and
the execution plan may comprise additional execution operators for data movement among platforms (\eg~\at{Broadcast}).
% , \ie~moving data from one platform to another.
In the next section, we give an overview of this component as well as how it transforms the k-means plan into an execution plan; and details of its functionality are presented in the subsequent sections.

\myparagraph{Cross-platform executor}
\rheem' executor orchestrates the execution of the generated execution plan on the selected platforms.
For that purpose, it has a decoupled platform-specific driver for each available processing platform.
In addition, this component monitors the health of the ongoing execution and collects statistics to improve the cost-model of the optimizer.

%Interested readers can refer to~\cite{rheem-system} for more details about the system and to Appendix~\ref{section:apps} for the code of our k-means example.
%Additionally, we explain the \rheem code for our k-means example in Appendix~\ref{section:apps}.


==> kmeans.tex <==
%!TEX root = main.tex

\jorge{can someone (Seb?) please provide this code?}
